Semantic and Expressive Variation in Image Captions Across Languages

Computer vision often treats human perception as homogeneous: an implicit assumption that visual stimuli are perceived similarly by everyone. This assumption is reflected in the way researchers collect datasets and train vision models. By contrast, literature in cross-cultural psychology and linguistics has provided evidence that people from different cultural backgrounds observe vastly different concepts even when viewing the same visual stimuli. In this paper, we study how these differences manifest themselves in vision-language datasets and models, using language as a proxy for culture. By comparing textual descriptions generated across 7 languages for the same images, we find significant differences in the semantic content and linguistic expression. When datasets are multilingual as opposed to monolingual, descriptions have higher semantic coverage on average, where coverage is measured using scene graphs, model embeddings, and linguistic taxonomies. For example, multilingual descriptions have on average 29.9% more objects, 24.5% more relations, and 46.0% more attributes than a set of monolingual captions. When prompted to describe images in different languages, popular models (e.g. LLaVA) inherit this bias and describe different parts of the image. Moreover, finetuning models on captions from one language performs best on corresponding test data from that language, while finetuning on multilingual data performs consistently well across all test data compositions. Our work points towards the need to account for and embrace the diversity of human perception in the computer vision community.

==> sec/_1_commands.tex <==
\newcommand\andre[1]{{\color{brown}[{#1}]$_{-\text{Andre}}$}}
\newcommand\seb[1]{{\color{orange}[{#1}]$_{-\text{Seb}}$}}
\newcommand\rk[1]{{\color{blue}[{#1}]$_{-\text{Ranjay}}$}}
\newcommand\matt[1]{{\color{green}[{#1}]$_{-\text{matt}}$}}
% \newcommand\todo[1]{{\color{red}[{#1}]$_{-\text{TODO}}$}}

% \newcommand\attention[1]{{\color{red}$^{\mathbf{!}}$[{#1}]}}
\newcommand\attention[1]{{}}
\newcommand*\rot{\rotatebox{90}}

\definecolor{lightgray}{gray}{0.9}
\definecolor{gold}{HTML}{ffccbc}
\definecolor{silver}{HTML}{ffecb3}

% \definecolor{one}{HTML}{f8bbd0}
% \definecolor{two}{HTML}{d1c4e9}
% \definecolor{three}{HTML}{eeeeee}

\newcommand{\first}[1]{\tcbox[on line,colframe=gold,boxsep=0pt,left=0.5pt,right=0.5pt, enlarge top by=0.005cm, enlarge bottom by=0.005cm, arc=0.4pt, top=0.3pt,bottom=0.3pt,colback=gold]{#1}}

\newcommand{\second}[1]{\tcbox[on line,colframe=silver,boxsep=0pt,left=0.7pt,right=0.7pt, enlarge top by=0.005cm, enlarge bottom by=0.005cm, arc=0.4pt, top=0.3pt,bottom=0.3pt,colback=silver]{#1}}


\newcommand\one[1]{{#1}}
\newcommand\two[1]{{#1}}
\newcommand\three[1]{{#1}}

% \definecolor{labbg}{HTML}{bdbdbd}
% % \definecolor{labborder}{RGB}{115, 20, 12}
% \newtcbox{\circled}[1][]{enhanced,
%  box align=base,
%  nobeforeafter,
%  colback=labbg,
%  colframe=labbg,
%  size=small,
%  fontupper=\scriptsize\bf\sffamily,
%  left=0.5pt,
%  right=0.5pt,
%  top=0.5pt,
%  bottom=0.5pt,
%  boxsep=2pt,
%  arc=4.5pt,
%  #1}


\newcommand{\circled}[1]{%
  \tikz[baseline=(char.base)]{
    \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

% \newcommand{\first}[1]{\tcbox[on line,colframe=gold,boxsep=0pt,left=0.5pt,right=0.5pt, enlarge top by=0.005cm, enlarge bottom by=0.005cm, arc=0.4pt, top=0.3pt,bottom=0.3pt,colback=gold]{#1}}

% \newcommand{\second}[1]{\tcbox[on line,colframe=silver,boxsep=0pt,left=0.7pt,right=0.7pt, enlarge top by=0.005cm, enlarge bottom by=0.005cm, arc=0.4pt, top=0.3pt,bottom=0.3pt,colback=silver]{#1}}

% \newcommand{\three}[1]{\tcbox[on line,colframe=three,boxsep=0pt,left=2pt,right=2pt, enlarge top by=0.005cm, enlarge bottom by=0.005cm, arc=1pt, top=1pt,bottom=1pt,colback=three]{#1}}

==> tables/main-table-2.tex <==
\begin{table}[htbp]
\centering
\caption{Primary results across evaluations.}
\label{your-table-label}
\scriptsize
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Level} & \multicolumn{3}{|c|}{Language-centric} \\ \hline
\textbf{Eval} & \multicolumn{3}{|c|}{Logical meaning} \\ \hline
\textbf{Source} & \multicolumn{3}{|c|}{Vertex} \\ \hline
\textbf{Metric} & Obj & Attr & Rel \\ \hline
\textbf{en} & ... & ... & ... \\ \hline
\textbf{fr} & ... & ... & ... \\ \hline
\textbf{de} & ... & ... & ... \\ \hline
\textbf{ru} & ... & ... & ... \\ \hline
\textbf{zh} & ... & ... & ... \\ \hline
\textbf{ja} & ... & ... & ... \\ \hline
\textbf{ko} & ... & ... & ... \\ \hline
\textbf{en,fr,zh} & ... & ... & ... \\ \hline
\textbf{fr,zh,ru} & ... & ... & ... \\ \hline
\textbf{zh,ja,ko} & ... & ... & ... \\ \hline
\textbf{multi} & ... & ... & ... \\ \hline
\end{tabular}
\vspace{0.5cm}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Perspective} & Language-centric & Language-centric & Language-centric \\ \hline
\textbf{Evaluation} & Syntactic expression & Syntactic expression & Syntactic expression \\ \hline
\textbf{Data Source} & Vertex & Vertex & Vertex \\ \hline
\textbf{Metric} & Concreteness & Analytic & Clout \\ \hline
\textbf{en} & ... & ... & ... \\ \hline
\textbf{fr} & ... & ... & ... \\ \hline
\textbf{de} & ... & ... & ... \\ \hline
\textbf{ru} & ... & ... & ... \\ \hline
\textbf{zh} & ... & ... & ... \\ \hline
\textbf{ja} & ... & ... & ... \\ \hline
\textbf{ko} & ... & ... & ... \\ \hline
\textbf{en,fr,zh} & ... & ... & ... \\ \hline
\textbf{fr,zh,ru} & ... & ... & ... \\ \hline
\textbf{zh,ja,ko} & ... & ... & ... \\ \hline
\textbf{multi} & ... & ... & ... \\ \hline
\end{tabular}
\vspace{0.5cm}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Perspective} & Model-centric & Model-centric & Model-centric \\ \hline
\textbf{Evaluation} & Embeddings & Embeddings & Embeddings \\ \hline
\textbf{Data Source} & Vertex & Vertex & Vertex \\ \hline
\textbf{Metric} & Semantic coverage & Semantic coverage & Semantic coverage \\ \hline
\textbf{en} & ... & ... & ... \\ \hline
\textbf{fr} & ... & ... & ... \\ \hline
\textbf{de} & ... & ... & ... \\ \hline
\textbf{ru} & ... & ... & ... \\ \hline
\textbf{zh} & ... & ... & ... \\ \hline
\textbf{ja} & ... & ... & ... \\ \hline
\textbf{ko} & ... & ... & ... \\ \hline
\textbf{en,fr,zh} & ... & ... & ... \\ \hline
\textbf{fr,zh,ru} & ... & ... & ... \\ \hline
\textbf{zh,ja,ko} & ... & ... & ... \\ \hline
\textbf{multi} & ... & ... & ... \\ \hline
\end{tabular}
\vspace{0.5cm}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Perspective} & Model-centric & Model-centric & Model-centric \\ \hline
\textbf{Evaluation} & Fine-tuning & Fine-tuning & Fine-tuning \\ \hline
\textbf{Data Source} & Vertex & Vertex & Vertex \\ \hline
\textbf{Metric} & FT on English & FT on French & FT on German \\ \hline
\textbf{en} & ... & ... & ... \\ \hline
\textbf{fr} & ... & ... & ... \\ \hline
\textbf{de} & ... & ... & ... \\ \hline
\textbf{ru} & ... & ... & ... \\ \hline
\textbf{zh} & ... & ... & ... \\ \hline
\textbf{ja} & ... & ... & ... \\ \hline
\textbf{ko} & ... & ... & ... \\ \hline
\textbf{en,fr,zh} & ... & ... & ... \\ \hline
\textbf{fr,zh,ru} & ... & ... & ... \\ \hline
\textbf{zh,ja,ko} & ... & ... & ... \\ \hline
\textbf{multi} & ... & ... & ... \\ \hline
\end{tabular}
\end{table}


% \begin{table}[htbp]
% \centering
% \caption{Primary results across evaluations.}
% \label{your-table-label}
% \scriptsize
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \textbf{Level} & \multicolumn{3}{|c|}{Language-centric} & \multicolumn{3}{|c|}{Syntactic expression} & \multicolumn{3}{|c|}{Embeddings} & \multicolumn{3}{|c|}{Fine-tuning} \\ \hline
% \textbf{Eval} & \multicolumn{3}{|c|}{Logical meaning} & \multicolumn{3}{|c|}{Concreteness} & \multicolumn{3}{|c|}{Semantic coverage} & \multicolumn{3}{|c|}{FT on English} \\ \hline
% \textbf{Source} & \multicolumn{3}{|c|}{Vertex} & \multicolumn{3}{|c|}{Vertex} & \multicolumn{3}{|c|}{Vertex} & \multicolumn{3}{|c|}{Vertex} \\ \hline
% \textbf{Metric} & Obj & Attr & Rel & Obj & Attr & Rel & Obj & Attr & Rel & Obj & Attr & Rel \\ \hline
% \textbf{en} & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% \textbf{fr} & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% \textbf{de} & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% \textbf{ru} & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% \textbf{zh} & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% \textbf{ja} & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% \textbf{ko} & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% \textbf{en,fr,zh} & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% \textbf{fr,zh,ru} & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% \textbf{zh,ja,ko} & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% \textbf{multi} & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
% \end{tabular}
% \end{table}


==> tables/old-table-2.tex <==
% metrics are normally read vertically, and different hyps tested across the rows
% break up tables and make it easier to see what ppl should be paying attentino to
% break up tables and transpose (language combos as rows and metrics as columns)
% probably don't need cell shading after breakin gup and transposing


\begin{sidewaystable}
\scriptsize
\centering
\caption{Primary results across each of four evaluations. Shaded comparisons emphasize comparison between monolingual English caption sets and multilingual caption sets (including English and other languages), which have higher coverage/diversity across their respect evaluations.}
\label{primary-table}

\begin{tabular}{|c|c|c|c|r|r|r|r|r|r|r|r|r|r|r|}
\hline
\multirow{2}{*}{\textbf{Level}} & \multirow{2}{*}{\textbf{Evaluation}} & \multirow{2}{*}{\textbf{Data Source}} & \multirow{2}{*}{\textbf{Metric}} & \multicolumn{7}{c|}{\textbf{Monolingual}} & \multicolumn{4}{c|}{\textbf{Multilingual}} \\ 
\cline{5-15}
& & & & \textbf{en} & \textbf{fr} & \textbf{de} & \textbf{ru} & \textbf{zh} & \textbf{ja} & \textbf{ko} & \textbf{en,fr,zh} & \textbf{fr,zh,ru} & \textbf{de,fr,ru} & \textbf{multi}\footnote{The `multi' column is computed by randomly sampling across all languages.} \\ 
\hline
\multirow{21}{*}{Language} & \multirow{6}{*}{Logical meaning} & \multirow{3}{*}{Vertex} & Objects & 3.65 & 3.51 & 3.60 & 3.86 & 3.46 & 3.13 & 3.18 & 4.13 & 4.24 & 4.13 & 4.17 \\
\cline{4-15}
& & & Relations & 2.96 & 2.83 & 2.89 & 3.20 & 2.68 & 2.37 & 2.47 & 3.45 & 3.48 & 3.38 & 3.40 \\
\cline{4-15}
& & & Attributes & 1.67 & 1.67 & 1.79 & 1.86 & 1.66 & 1.59 & 1.62 & 2.29 & 2.40 & 2.33 & 2.33 \\
\cline{3-15}
& & \multirow{3}{*}{LLaVA} & Objects & 4.54 & 5.05 & 5.26 & 4.52 & 4.54 & - & \footnote{Korean is excluded from LLaVA results due to extremely poor caption generation in the language.} - & 6.14 & 6.15 & 6.25 & 5.93 \\
\cline{4-15}
& & & Relations & 3.79 & 4.21 & 4.42 & 3.67 & 3.66 & - & - & 4.85 & 4.76 & 4.97 & 4.54  \\
\cline{4-15}
& & & Attributes & 2.75 & 3.47 & 3.50 & 2.76 & 3.25 & - & - & 4.00 & 3.99 & 4.07 & 3.86 \\
\cline{2-15}
& & \multirow{3}{*}{XM} & Objects & 2.59 & 2.92 & 3.16 & 3.03 & 2.99 & 3.41 & 2.71 & 3.71 & 3.92 & 3.93 & 4.35 \\
\cline{4-15}
& & & Relations & 1.54 & 1.76 & 1.94 & 1.88 & 1.71 & 1.99 & 1.59 & 2.41 & 2.57 & 2.57 & 2.94 \\
\cline{4-15}
& & & Attributes & 1.27 & 1.66 & 1.97 & 1.74 & 2.01 & 2.47 & 1.46 & 2.36 & 2.59 & 2.55 & 2.97 \\
\hline
& \multirow{15}{*}{Expression} & \multirow{5}{*}{Vertex} & Concreteness & 1.64 & 1.64 & 1.67 & 1.66 & 1.51 & 1.50 & 1.56 & 1.75 & 1.74 & 1.73 & 1.81 \\
\cline{4-15}
& &  & Analytic & 0.85 & 0.43 & 0.62 & 1.08 & 2.3 & 2.6 & 2.17 & 2.02 & 2.05 & 1.0 & 2.3 \\
\cline{4-15}
& & & Clout & 4.94 & 5.05 & 5.40 & 7.14 & 6.92 & 6.49 & 5.56 & 10.59 & 11.29 & 9.8 & 11.01 \\
\cline{4-15}
& & & Authentic & 23.21 & 22.8 & 21.68 & 23.07 & 23.51 & 25.01 & 21.67 & 40.16 & 36.94 & 31.85 & 38.06 \\
\cline{4-15}
& & & Tone & 1.85 & 1.84 & 2.03 & 2.63 & 2.05 & 1.96 & 2.05 & 3.98 & 4.10 & 4.19 & 3.92 \\
\cline{3-15}
& & \multirow{5}{*}{LLaVA} & Concreteness & 2.17 & 2.44 & 2.53 & 2.27 & 2.33 & - & - & 2.54 & 2.54 & 2.57 & 2.56 \\
\cline{4-15}
& &  & Analytic & 2.85 & 4.64 & 14.72 & 7.53 & 23.05 & - & - & 22.03 & 22.29 & 23.76 & 19.61 \\
\cline{4-15}
& & & Clout & 14.19 & 19.96 & 15.81 & 23.15 & 21.3 & 29.57 & & 23.06 & 26.78 & 26.84 & 28.72 \\
\cline{4-15}
& & & Authentic & 35.97 & 38.01 & 34.33 & 37.20 & 44.63 & 42.92 & & 54.94 & 54.64 & 54.82 & 53.15 \\
\cline{4-15}
& & & Tone & 6.79 & 9.53 & 16.64 & 16.48 & 11.56 & 9.55 & & 16.74 & 20.79 & 19.80 & 16.56 \\
\cline{3-15}
& & \multirow{5}{*}{XM} & Concreteness & 1.80 & 2.24 & 2.11 & 2.03 & 2.26 & 2.25 & 2.14 & 2.08 & 2.13 & 2.10 & 2.17\\
\cline{4-15}
& &  & Analytic & 1.88 & 2.31 & 1.62 & 0.76 & 5.02 & 5.28 & 5.13 & 4.12 & 4.37 & 4.47 & 4.49 \\
\cline{4-15}
& & & Clout & 9.66 & 14.77 & 15.00 & 14.14 & 13.32 & 13.10 & 12.24 & 18.8 & 20.51 & 19.54 & 19.39 \\
\cline{4-15}
& & & Authentic & 33.21 & 40.09 & 42.22 & 32.35 & 34.02 & 33.83 & 35.28 & 53.12 & 54.41 & 53.35 & 53.21 \\
\cline{4-15}
& & & Tone & 8.62 & 12.16 & 9.74 & 10.90 & 10.59 & 9.18 & 9.07 & 13.78 & 14.69 & 15.42 & 15.40 \\
\hline

\multirow{6}{*}{Model} & \multirow{3}{*}{Embeddings} & Vertex & \multirow{3}{*}{Coverage} & 0.19 & 0.18 & 0.19 & 0.22 & 0.20 & 0.19 & 0.37 & 0.37 & 0.33 & 0.38 & 0.49 \\
\cline{3-3}
\cline{5-15}
& & LLaVA & & 0.22 & 0.29 & 0.28 & 0.29 & 0.36 & 0.40 && 0.45 & 0.47 & 0.43 & 0.47 \\
\cline{3-3}
\cline{5-15}
& & XM & & 0.38 & 0.0.42 & 0.43 & 0.40 & 0.46 & 0.42 & 0.43 & 0.54 & 0.54 & 0.49 & 0.52  \\
\cline{2-15}

& \multirow{3}{*}{Fine-tuning} & Vertex & \multirow{3}{*}{Best Model}\footnote{Each cell value is the original language of the caption set used to train the model which performed best as evaluated by the caption set originally from the language specified in the column.} & en & de & fr & ru & zh & ja & ko & & & & multi \\
\cline{3-3}
\cline{5-15}
& & LLaVA & & en & de & fr & ru & zh & ja &  & & & & multi \\
\cline{3-3}
\cline{5-15}
& & XM & & en & de & fr & ru & zh & ja & ko & & & & multi \\
% \cline{4-15}
% & & & FT on French &  0.248 & 0.240 & \first{0.259} & 0.234 & 0.236 & 0.239 & 0.253 & & & & 0.246 \\
% \cline{4-15}
% & & & FT on German & 0.213 & \first{0.245} & 0.219 & 0.217 & 0.215 & 0.210 & 0.226 & & & & 0.219 \\
% \cline{4-15}
% & & & FT on Russian & 0.226 & 0.234 & 0.228 & \first{0.254} & 0.231 & 0.236 & 0.237 & & & & 0.239 \\
% \cline{4-15}
% & & & FT on Chinese & 0.199 & 0.202 & 0.199 & 0.207 & \first{0.247} & 0.220 & 0.224 & & & & 0.216 \\
% \cline{4-15}
% & & & FT on Japanese & 0.212 & 0.212 & 0.215 & 0.212 & 0.226 & \first{0.266} & 0.245 & & & & 0.223 \\
% \cline{4-15}
% & & & FT on Korean & 0.218 & 0.222 & 0.224 & 0.217 & 0.242 & 0.239 & \first{0.271} & & & & 0.235 \\
% \cline{4-15}
% & & & FT on multi & \second{0.239} & \second{0.233} & \second{0.234} & \second{0.233} & \second{0.235} & \second{0.243} & \second{0.252} & & & & \second{0.244} \\
\hline
\end{tabular}
\end{sidewaystable}



==> tables/old-table.tex <==
\begin{sidewaystable}
\scriptsize
\centering
\caption{Primary results across each of four evaluations. Shaded comparisons emphasize comparison between monolingual English caption sets and multilingual caption sets (including English and other languages), which have higher coverage/diversity across their respect evaluations.}
\label{primary-table}

\begin{tabular}{|c|c|c|c|>{\columncolor{lightgray}}r|r|r|r|r|r|r|>{\columncolor{lightgray}}r|r|r|>{\columncolor{lightgray}}r|}
\hline
\multirow{2}{*}{\textbf{Level}} & \multirow{2}{*}{\textbf{Evaluation}} & \multirow{2}{*}{\textbf{Data Source}} & \multirow{2}{*}{\textbf{Metric}} & \multicolumn{7}{c|}{\textbf{Monolingual}} & \multicolumn{4}{c|}{\textbf{Multilingual}} \\ 
\cline{5-15}
& & & & \textbf{en} & \textbf{fr} & \textbf{de} & \textbf{ru} & \textbf{zh} & \textbf{ja} & \textbf{ko} & \textbf{en,fr,zh} & \textbf{fr,zh,ru} & \textbf{de,fr,ru} & \textbf{multi} \\ 
\hline
\multirow{21}{*}{Language} & \multirow{6}{*}{Logical meaning} & \multirow{3}{*}{Vertex} & Objects & 3.65 & 3.51 & 3.60 & 3.86 & 3.46 & 3.13 & 3.18 & 4.13 & 4.25 & &  \\
\cline{4-15}
& & & Relations & 2.96 & 2.83 & 2.89 & 3.20 & 2.68 & 2.37 & 2.47 & 3.60 & 3.56 & & \\
\cline{4-15}
& & & Attributes & 1.67 & 1.67 & 1.79 & 1.86 & 1.66 & 1.59 & 1.62 & 2.13 & 2.15 & & \\
\cline{3-15}
& & \multirow{3}{*}{LLaVA} & Objects & 4.54 & 5.05 & 5.26 & 4.52 & 4.54 & 3.32 & & 5.87 & 6.02 & & \\
\cline{4-15}
& & & Relations & 3.79 & 4.21 & 4.42 & 3.67 & 3.66 & 2.40 & & 4.84 & 4.97 & & \\
\cline{4-15}
& & & Attributes & 2.75 & 3.47 & 3.50 & 2.76 & 3.25 & 2.70 & & 4.10 & 4.07 & & \\
\cline{2-15}
& \multirow{15}{*}{Syntactic expression} & \multirow{5}{*}{Vertex} & Concreteness & 32.80 & 32.60 & 33.40 & 33.20 & 30.20 & 30.00 & 31.20 & 35.80 & & & 46.60 \\
\cline{4-15}
& &  & Analytic & 0.84 & 0.43 & 0.62 & 1.08 & 2.30 & 2.60 & 2.17 & 2.08 & & & 7.95 \\
\cline{4-15}
& & & Clout & 4.94 & 5.05 & 5.4 & 7.14 & 6.92 & 6.49 & 5.56 & 11.16 & & & 27.15 \\
\cline{4-15}
& & & Authentic & 23.21 & 22.8 & 21.68 & 23.07 & 23.51 & 25.01 & 21.67 & 39.5 & & & 76.47 \\
\cline{4-15}
& & & Tone & 1.85 & 1.84 & 2.03 & 2.63 & 2.05 & 1.96 & 2.05 & 4.33 & & & 10.18 \\
\cline{3-15}
& & \multirow{5}{*}{LLaVA} & Concreteness & 2.17 & 2.53 & 2.44 & 2.27 & 2.33 & 2.21 & & & & & 3.19 \\
\cline{4-15}
& &  & Analytic & 2.85 & 4.64 & 14.72 & 7.53 & 23.05 & 20.86 & & & & & 18.09 \\
\cline{4-15}
& & & Clout & 14.19 & 19.96 & 15.81 & 23.15 & 21.3 & 29.57 & & & & & 29.14 \\
\cline{4-15}
& & & Authentic & 35.97 & 38.01 & 34.33 & 37.20 & 44.63 & 42.92 & & & & & 52.59 \\
\cline{4-15}
& & & Tone & 6.79 & 9.53 & 16.64 & 16.48 & 11.56 & 9.55 & & & & & 16.56 \\
\cline{3-15}
& & \multirow{5}{*}{XM} & Concreteness & 36.06 & 44.74 & 42.16 & 40.51 & 45.13 & 44.90 & 42.70 & & & & 43.28 \\
\cline{4-15}
& &  & Analytic & 1.88 & 2.31 & 1.62 & 0.76 & 5.02 & 5.28 & 5.13 &   & & & 4.66 \\
\cline{4-15}
& & & Clout & 9.66 & 14.77 & 15.00 & 14.14 & 13.32 & 13.10 & 12.24 & & & & 19.66 \\
\cline{4-15}
& & & Authentic & 33.21 & 40.09 & 42.22 & 32.35 & 34.02 & 33.83 & 35.28 & & & & 51.87 \\
\cline{4-15}
& & & Tone & 8.62 & 12.16 & 9.74 & 10.90 & 10.59 & 9.18 & 9.07 & & & & 13.88 \\
\hline
\multirow{6}{*}{Model} & \multirow{3}{*}{Embeddings} & Vertex & \multirow{3}{*}{Coverage} & 0.19 & 0.18 & 0.19 & 0.22 & 0.20 & 0.19 & 0.21 & 0.37 & 0.37 & 0.38 & \\
\cline{3-3}
\cline{5-15}
& & LLaVA & & 0.22 & 0.29 & 0.28 & 0.29 & 0.36 & 0.40 && 0.45 & 0.47 & 0.46 & \\
\cline{3-3}
\cline{5-15}
& & XM & & 0.38 & 0.40 & 0.38 & 0.40 & 0.45 & 0.42 & 0.41 & 0.41 & 0.46 & 0.45 &  \\
\cline{2-15}
& \multirow{3}{*}{Fine-tuning} & Vertex & \multirow{3}{*}{Best Model}\footnote{Each cell value is the original language of the caption set used to train the model which performed best as evaluated by the caption set originally from the language specified in the column.} & en & de & fr & ru & zh & ja & ko & & & & multi \\
\cline{3-3}
\cline{5-15}
& & LLaVA & & en & de & fr & ru & zh & ja &  & & & & multi \\
\cline{3-3}
\cline{5-15}
& & XM & & en & de & fr & ru & zh & ja & ko & & & & multi \\
% \cline{4-15}
% & & & FT on French &  0.248 & 0.240 & \first{0.259} & 0.234 & 0.236 & 0.239 & 0.253 & & & & 0.246 \\
% \cline{4-15}
% & & & FT on German & 0.213 & \first{0.245} & 0.219 & 0.217 & 0.215 & 0.210 & 0.226 & & & & 0.219 \\
% \cline{4-15}
% & & & FT on Russian & 0.226 & 0.234 & 0.228 & \first{0.254} & 0.231 & 0.236 & 0.237 & & & & 0.239 \\
% \cline{4-15}
% & & & FT on Chinese & 0.199 & 0.202 & 0.199 & 0.207 & \first{0.247} & 0.220 & 0.224 & & & & 0.216 \\
% \cline{4-15}
% & & & FT on Japanese & 0.212 & 0.212 & 0.215 & 0.212 & 0.226 & \first{0.266} & 0.245 & & & & 0.223 \\
% \cline{4-15}
% & & & FT on Korean & 0.218 & 0.222 & 0.224 & 0.217 & 0.242 & 0.239 & \first{0.271} & & & & 0.235 \\
% \cline{4-15}
% & & & FT on multi & \second{0.239} & \second{0.233} & \second{0.234} & \second{0.233} & \second{0.235} & \second{0.243} & \second{0.252} & & & & \second{0.244} \\
\hline
\end{tabular}
\end{sidewaystable}



==> tables/semantic.tex <==
\begin{table}
    \centering
    \begin{tabular}{cc|ccc|ccc}
         \multicolumn{2}{c|}{\textit{Caption Source}} & \multicolumn{3}{c|}{Vertex} & \multicolumn{3}{c|}{LLaVA} \\
         \cline{1-8}
         \multicolumn{2}{c|}{\textit{Metric}} & Obj.s & Rel.s & Attr.s & Obj.s & Rel.s & Attr.s \\
         \hline
        \multirow{7}{*}{\rotatebox{90}{Mono}} & en & 3.65 & 2.96 & 1.67 & 4.54 & 3.79 & 2.75 \\
        & fr & 3.51 & 2.83 & 1.67 & 5.05 & 4.21 & 3.47 \\
        & de & 3.60 & 2.89 & 1.79 & 5.26 & 4.42 & 3.50 \\
        & ru & 3.86 & 3.20 & 1.86 & 4.52 & 3.67 & 2.76 \\
        & zh & 3.46 & 2.68 & 1.66 & 4.54 & 3.66 & 3.25 \\
        & ja & 3.13 & 2.37 & 1.59 & 3.32 & 2.40 & 2.70 \\
        & ko & 3.18 & 2.47 & 1.62 & - & - & - \\
        \hline
        \multirow{4}{*}{\rotatebox{90}{Multi}} & en,fr,zh & 4.13 & 3.45 & 2.29 & 6.14 & 4.85 & 4.00 \\
        & fr,zh,ru & 4.24 & 3.48 & 2.40 & 6.15 & 4.76 & 3.99 \\
        & de,fr,ru & 4.13 & 3.38 & 2.33 & 6.25 & 4.97 & 4.07 \\
        & avg & 4.17 & 3.40 & 2.33 & 5.93 & 4.54 & 3.86 \\
    \end{tabular}
    \caption{\textbf{Semantic evaluation results.} }
    \label{tab:my_label}
\end{table}


==> tables/syntactic.tex <==
\begin{table}
    \centering
    \begin{tabular}{cc|ccccc|ccccc|ccccc}
         \multicolumn{2}{c|}{\textit{Evaluation Metric}} & \multicolumn{5}{c|}{Vertex} & \multicolumn{5}{c|}{LLaVA} & \multicolumn{5}{c}{XM} \\
         \cline{1-17}
         \multicolumn{2}{c|}{\textit{Language / Combo}} & Conc. & Analy. & Clout & Auth. & Tone & Conc. & Analy. & Clout & Auth. & Tone & Conc. & Analy. & Clout & Auth. & Tone \\
         \hline
        \multirow{7}{*}{\rotatebox{90}{Mono}} & en & 1.64 & 0.85 & 4.94 & 23.21 & 1.85 & 2.17 & 2.85 & 14.19 & 35.97 & 6.79 & 1.80 & 1.88 & 9.66 & 33.21 & 8.62 \\
        & fr & 1.64 & 0.43 & 5.05 & 22.80 & 1.84 & 2.44 & 4.64 & 19.96 & 38.01 & 9.53 & 2.24 & 2.31 & 14.77 & 40.09 & 12.16 \\
        & de & 1.67 & 0.62 & 5.40 & 21.68 & 2.03 & 2.53 & 14.72 & 15.81 & 34.33 & 16.64 & 2.11 & 1.62 & 15.00 & 42.22 & 9.74 \\
        & ru & 1.66 & 1.08 & 7.14 & 23.07 & 2.63 & 2.27 & 7.53 & 23.15 & 37.20 & 16.48 & 2.03 & 0.76 & 14.14 & 32.35 & 10.90 \\
        & zh & 1.51 & 2.30 & 6.92 & 23.51 & 2.05 & 2.33 & 23.05 & 21.30 & 44.63 & 11.56 & 2.26 & 5.02 & 13.32 & 34.02 & 10.59 \\
        & ja & 1.50 & 2.60 & 6.49 & 25.01 & 1.96 & 2.21 & 20.86 & 29.57 & 42.92 & 9.55 & 2.25 & 5.28 & 13.10 & 33.83 & 9.18 \\
        & ko & 1.56 & 2.17 & 5.56 & 21.67 & 2.05 & - & - & - & - & - & 2.14 & 5.13 & 12.24 & 35.28 & 9.07 \\
        \hline
        \multirow{4}{*}{\rotatebox{90}{Multi}} & en,fr,zh & 1.75 & 2.02 & 10.59 & 40.16 & 3.98 & 2.54 & 22.03 & 23.06 & 54.94 & 16.74 & 2.08 & 4.12 & 18.8 & 53.12 & 13.78 \\
        & fr,zh,ru & 1.74 & 2.05 & 11.29 & 36.94 & 4.10 & 2.54 & 22.29 & 26.78 & 54.64 & 20.79 & 2.13 & 4.37 & 20.51 & 54.41 & 14.69 \\
        & de,fr,ru & 1.73 & 1.00 & 9.80 & 31.85 & 4.19 & 2.57 & 23.76 & 26.84 & 54.82 & 19.80 & 2.10 & 4.47 & 19.54 & 53.35 & 15.42 \\
        & avg & 1.81 & 2.30 & 11.01 & 38.06 & 3.92 & 2.56 & 19.61 & 28.72 & 53.15 & 16.56 & 2.17 & 4.49 & 19.39 & 53.21 & 15.40 \\
    \end{tabular}
    \caption{\textbf{Expression evaluation results including Vertex, LLaVA, and XM data.}}
    \label{tab:expression_evaluation_extended}
\end{table}

